CWTHF: Subhalo Identification with Continuous Wavelet Transform

With advances in cosmology and computer science, cosmological simulations now resolve structures in increasingly fine detail. As key tracers of hierarchical structure formation, subhalos are among the most important objects within these simulations. In our previous work, we established that the continuous wavelet transform (CWT) can effectively extract clustering information and serve as a robust halo finder. Here, we extend the CWT framework to subhalo identification by adapting the Continuous Wavelet Transform Halo Finder (CWTHF) code. This extension extends the unbinding procedure, which enables the reliable identification of gravitationally bound substructures. The algorithm identifies density peaks within known halos or subhalos and segments the surrounding volume accordingly. Once a new subhalo is registered, its position is recorded to prevent duplicate detection. We validate our approach using the TNG50-2 and TNG100-1 simulations, as well as a single Friends-of-Friends (FOF) halo, by comparing the resulting CWT catalog against the reference SUBFIND catalog. Because the method inherits the original computational framework, our subhalo finder maintains a favorable linear time complexity of $\mathcal{O}(N)$.

==> flowchart.tex <==
	\begin{figure}[t]  
		\scriptsize  
		\tikzstyle{format}=[rectangle,draw,thin,fill=blue!50!black!20, draw=none]  
		%定义语句块的颜色,形状和边
		\tikzstyle{test}=[diamond,aspect=2,draw,thin,fill=blue!50!black!20, draw=none]  
		%定义条件块的形状,颜色
		\tikzstyle{point}=[coordinate,on grid,]  
		%像素点,用于连接转移线
		\begin{tikzpicture}[scale=0.44]
        %[node distance=10mm,auto,>=latex',thin,start chain=going below,every join/.style={norm},] 
		%start chain=going below指明了流程图的默认方向，node distance=8mm则指明了默认的node距离。这些可以在定义node的时候更改，比如说 
		%\node[point,right of=n3,node distance=10mm] (p0){};  
		%这里声明了node p0，它在node n3 的右边，距离是10mm。{End the program}
		\node[rectangle,draw,thin,fill=blue!50!black!20,align=center, draw=none] (start){Initialize the program:\\
                                set the range of the $k_w$ \\
                                and scale resolution $N_w$};
		\node[format,below of=start,node distance=15mm](initi){$i = 1$};
  	\node[format,below of=initi,align=center,node distance=15mm](initgrid){
                                calculating\_grid = []\\
                                current\_grid = []};
		\node[test,below of=initgrid,node distance=20mm](circulate){$i \leq N_w$?};
		\node[format,left of=circulate,node distance=20mm](iplus1){
        $i=i+1$
        };
        \node[format,right of=circulate,node distance=40mm,align=center](last_iterate){
                                calculating\_grid = current\_grid\\
                                current\_grid = zero like array};
		\node[format,above of=last_iterate,align=center](haloseg2){Find all the local maxima in\\
                                calculating\_grid and segment the grid};     
		\node[format,above of=haloseg2,align=center,node distance=12mm](label2){Assign particles with no label\\
                                to the segmented grid and \\
                                label them temp ID};  \\ 
		\node[format,above of=label2,align=center](check2){
        Discard unphysical groups};    
		\node[format,above of=check2,align=center](updatelabel2){Store the particles that \\
                                 pass self-boundness check and\\
                                 label them with halo ID};   
		\node[rectangle,draw,thin,fill=blue!50!black!20,above of=updatelabel2,align=center, draw=none](end){Save labeled particles \\
                                 and stop the program};                                  
		\node[test,below of=circulate,node distance=15mm](checki){$i = 1$?};
		\node[format,below of=checki,node distance=15mm,align=center](setkw1){Select the $i$-th element \\
                                of $k_w$, $k_{w,i}$};
		\node[format,below of=setkw1,align=center](NgNw){$N_g$ = Int(400$k_{w,i}$+150)\\
                                $N_w$ = Int(1.5/$k_{w,i}$+5)};
		\node[format,below of=NgNw,align=center](gridCWT1){
        Assign particles to $N_g$\\
                                grid and calculate the grid CWT};
        \node[format,below of=gridCWT1,align=center](updategrid1){
                                calculating\_grid = current\_grid\\
                                current\_grid = ${\rm C}_i$};
		\node[point,below of=updategrid1,node distance=10mm](point1){};
        \node[point,left of=point1,node distance=20mm](point2){};
        \node[format,right of=checki,node distance=40mm,align=center](setkw2){Select the $i$-th element \\
                                of $k_w$, $k_{w,i}$};
		\node[format,below of=setkw2,align=center](NgNw2){$N_g$ = Int(400$k_{w,i}$+150)\\
                                $N_w$ = Int(1.5/$k_{w,i}$+5)};
		\node[format,below of=NgNw2,align=center](gridCWT2){
        Assign particles to $N_g$\\
                                grid and calculate the grid CWT};
        \node[format,below of=gridCWT2,align=center](updategrid2){
                                calculating\_grid = current\_grid\\
                                current\_grid = ${\rm C}_i$};
		\node[format,below of=updategrid2,align=center](haloseg){Find all the local maxima in\\
                                calculating\_grid and segment the grid};     
		\node[format,below of=haloseg,align=center,node distance=12mm](label){Assign particles with no label\\
                                to the segmented grid and \\
                                label them temp ID};  \\ 
		\node[format,below of=label,align=center](check){
        Discard unphysical groups};    
		\node[format,below of=check,align=center](updatelabel){Store the particles that \\
                                 pass self-boundness check and\\
                                 label them with halo ID};    
        \node[point,left of=updatelabel,node distance=60mm](point5){};
		%\node[format] (n0) at(4,4){A}; 直接指定位置 
		%定义完node之后进行连线,
		%\draw[->] (n0.south) -- (n1); 带箭头实线
		%\draw[-] (n0.south) -- (n1); 不带箭头实线
		%\draw[<->] (n0.south) -- (n1.north);   双箭头
		%\draw[<-,dashed] (n1.south) -- (n2.north); 带箭头虚线 
		%\draw[<-] (n0.south) to node{Yes} (n1.north);  带字,字在箭头方向右边
		%\draw[->] (n1.north) to node{Yes} (n0.south);  带字,字在箭头方向左边
		%\draw[->] (n1.north) to[out=60,in=300] node{Yes} (n0.south);  曲线
		%\draw[->,draw=red](n2)--(n1);  带颜色的线
		\draw[->] (start)--(initi);
        \draw[->] (initi)--(initgrid);
        \draw[->] (initgrid)--(circulate);
		\draw[->](circulate) --node[left, text=green!60!black!90]{Yes} (checki);
        \draw[->](circulate) --node[above, text=red]{No} (last_iterate);
        \draw[->](last_iterate) -- (haloseg2);
        \draw[->](haloseg2)--(label2);
        \draw[->](label2)--(check2);
        \draw[->](check2)--(updatelabel2);
        \draw[->](updatelabel2)--(end);
		\draw[->](checki)--node[left, text=green!60!black!90]{Yes} (setkw1);
		\draw[->](setkw1)--(NgNw);
		\draw[->](NgNw)--(gridCWT1);
        \draw[->](gridCWT1)--(updategrid1);
        \draw[->, rounded corners=2mm] (updategrid1) -- (point1) -- (point2);
        \draw[->](point2)--(iplus1);
        \draw[->](iplus1)--(circulate);
        \draw[->](checki)--node[above, text=red]{No} (setkw2);
		\draw[->](setkw2)--(NgNw2);
		\draw[->](NgNw2)--(gridCWT2);
        \draw[->](gridCWT2)--(updategrid2);
        \draw[->](updategrid2)--(haloseg);
        \draw[->](haloseg)--(label);
        \draw[->](label)--(check);
        \draw[->](check)--(updatelabel);
        \draw[-, rounded corners=2mm](updatelabel)--(point5)--(point2);
		\end{tikzpicture}  
        \caption{The flowchart of the logical methodology of our CWTHF program. In this flowchart, we use the default values of the parameters as detailed in Section~\ref{sec:parameters}.}
        \label{approach_flowchart}
	\end{figure} 
